Evolutionary Multi-Task Injection Testing on Web Application Firewalls

Web application firewall (WAF) plays an integral role nowadays to protect web applications from various malicious injection attacks such as SQL injection, XML injection, and PHP injection, to name a few. However, given the evolving sophistication of injection attacks and the increasing complexity of tuning a WAF, it is challenging to ensure that the WAF is free of injection vulnerabilities such that it will block all malicious injection attacks without wrongly affecting the legitimate message. Automatically testing the WAF is, therefore, a timely and essential task. In this paper, we propose DaNuoYi, an automatic injection testing tool that simultaneously generates test inputs for multiple types of injection attacks on a WAF. Our basic idea derives from the cross-lingual translation in the natural language processing domain. In particular, test inputs for different types of injection attacks are syntactically different but may be semantically similar. Sharing semantic knowledge across multiple programming languages can thus stimulate the generation of more sophisticated test inputs and discovering injection vulnerabilities of the WAF that are otherwise difficult to find. To this end, in DaNuoYi, we train several injection translation models by using multi-task learning that translates the test inputs between any pair of injection attacks. The model is then used by a novel multi-task evolutionary algorithm to co-evolve test inputs for different types of injection attacks facilitated by a shared mating pool and domain-specific mutation operators at each generation. We conduct experiments on three real-world open-source WAFs and six types of injection attacks, the results reveal that DaNuoYi generates up to 3.8x and 5.78x more valid test inputs (i.e., bypassing the underlying WAF) than its state-of-the-art single-task counterparts and the context-free grammar-based injection construction.

==> cfg_tree.tex <==

\begin{figure*}
	\begin{minipage}[thtbp]{0.25\linewidth}
		\centering
	\tikzstyle{every node}=[
	  draw=black,thin,anchor=west, minimum height=2.5em]
	\tikzset{
		every node/.style={
			draw=black,thin,anchor=west, minimum height=2.5em}
	}
	
	\begin{tikzpicture}[
		supervisor/.style={%
			edge from parent fork down,
			level distance=2.5cm,
			text centered, text width=5cm},
		teammate/.style={%
			text centered, text width=3cm,
			level distance=2.5cm,
			fill=gray!10},
		subordinate/.style={%
			grow=down, xshift=-1.1cm, % Horizontal position of the child node
			text centered, text width=3cm,
			edge from parent path={
				(\tikzparentnode.205) |- (\tikzchildnode.west)
		}},
		level1/.style ={level distance=1.5cm},
		level2/.style ={level distance=3cm},
		level3/.style ={level distance=4.5cm},
		level4/.style ={level distance=6cm},
		level5/.style ={level distance=7.5cm},
		level 1/.style={sibling distance=4cm},
		level 1/.append style={level distance=4.5cm}]
		% \draw[help lines] (0,0) grid (4,3);
		
		% Supervisor
		\node [anchor=south, supervisor]
		{Supervisor\\Supervisory position\\Location}
		[edge from parent fork down]

    		% Teammate and Subordinates
    		child{node [teammate] {Teammate1\\Position1\\Location1}
    			child [subordinate,level1]
    			{node {Subordinate\\Position1\\Location1}}
    			child [subordinate,level2]
    			{node {Subordinate2}}
    			child [subordinate,level3]
    			{node {Subordinate3}}
    			child [subordinate,level4]
    			{node {Subordinate4\\Position4\\Location4}}
    			child [subordinate,level5]
    			{node {Subordinate5\\Position5\\Location5}}}
    		child{node [teammate] {Teammate2\\Position2\\Location2}
    			child[subordinate,level1]
    			{node {Subordinate1}}
    			child[subordinate,level2]
    			{node {Subordinate2}}
    			child[subordinate,level3]
    			{node {Third\\Teammate}}
    			child[subordinate,level4]
    			{node {Longtext-\\teammate}}}
    		child{node [teammate] {Teammate3\\Position3\\Location3}
    			child[subordinate,level1]
    			{node {Subordinate\\two lines}}
    			child[subordinate,level2]
    			{node {Subordinate2}}     
    			child[subordinate,level3]
    			{node {Subordinate3}}}
    		child{node [teammate] {Teammate4\\Position4\\Location4}
    			child[subordinate,level1]
    			{node {Subordinate1}}
    			child[subordinate,level2]
    			{node {Subordinate2}}}
    		child{node [teammate] {Teammate5\\Position5\\Location5}
    			child[subordinate,level1]
    			{node {First\\Subordinate}}
    			child[subordinate,level2]
    			{node {Subordinate2}}
    			child[subordinate,level3]
    			{node {Third\\Teammate}}
    			child[subordinate,level4]
    			{node {Longtext-\\teammate}}};
			
	\end{tikzpicture}

	\end{minipage}%
	\caption{An illustrative example of the grammar tree for XSS.}
	\label{fig:xss_grammar}
\end{figure*}

==> methods.tex <==
%!TeX root=main.tex

\section{Methodology}
\subsection{Data Sets}
We collected data from five large configurable systems. These configurable systems are the most popular and widely used in industry. These systems are briefly described in the following sections.\\
\emph{LLVM} The LLVM project is a modular, reusable collection of compiler and toolchain technologies. It provides a modern, SSA-based compilation strategy that supports both static and dynamic compilation of any programming language. LLVM has grown into a large project consisting of many subprojects, many of which are used in production by a wide range of commercial and open source projects, and widely used in academic research. LLVM has more than 578 officially provided configuration options (PASSs), and we extracted 20 configurations associated with performance, all of which are binary configurations. Using the 13 test-suits provided by Polybench, these tests are coded implementations of mathematical formulas with varying computational complexity. We collected two features as indicators to evaluate LLVM, one is the time to run the compiled executable test-suit and the size of the executable.\\
\emph{X264} X264 is a free, powerful audio stream encoding software. It offers the best performance, compression features, quality and visual optimization in its class. It also supports features needed for many different applications, such as TV broadcasts, Blu-ray low-latency video applications, and Web video. X264 forms the core of many online video services such as YouTube, Facebook, Vimeo and Hulu. It is widely used by TV broadcasters and ISPs. X264 provides a large number of parameter configurations to encode videos of different types and formats. Among more than 70 official configurations, we selected 17 configurations closely related to performance for data collection. Through the input of videos of different types and formats, the purpose of running in different running-environments was achieved. Our input videos range from 5M to 7G, and are available in a variety of formats. We use PSNR and SSIM, the most widely used image quality metrics, to evaluate the encoded video quality as a performance indicator for X264.\\
\emph{LRZIP} Long Range Zip (or LZMA RZIP) is an optimized compression program for large files. It consists of an RZIP step for redundancy reduction extensions and a normal compression program (LZMA, LZO, GZIP, BZIP2, or ZPAQ) step. The larger the file, the more space you can save by compression optimization, especially if the file is larger than 100MB. The software also provides different configurations to implement different optimized compression strategies. A total of 15 of these configurations are used for compression policies. We input different files from 2KB to 7G to collect the compression rate and compression duration of LRZIP in different file sizes and different configurations to show the performance of the software in different runn-environments.\\
\emph{APACHE} The Apache HTTP Server Project aims to provide a secure, efficient, and scalable server that provides HTTP services in sync with current HTTP standards. The Apache HTTP Server Project aims to develop and maintain open source HTTP servers for modern operating systems, including UNIX and Windows. Apache HTTP Server has multiple modules, of which the core module has 89 configurations and 21 MPM configurations, not to mention a variety of other small module configurations, and we collected data using the 15 configurations most associated with Apache performance. Apache Benchmark is used to obtain the performance indicators of the software system, among which one of the main indicators is the request handling capacity per unit time. The running-environment is set up by AB changing the total data flow and changing the parallel data flow.\\
\emph{SQLITE} SQLite is an embedded SQL database engine. Unlike most other SQL databases, SQLite does not have a separate server process. SQLite reads and writes directly to ordinary disk files. A complete SQL database with multiple tables, indexes, triggers, and views is contained in a single disk file. The configuration options for SQLite include compile-time configuration and runtime configuration. We extracted 18 of these key configurations, used LevelDB's Benchmark for data collection, and collected 14 of the target properties as SQLite performance metrics. The different running-environment refers to different running environments achieved by changing the total items of data accessed and the value size of data accessed in Benchmark.\\
\subsection{Search Algorithm}

\subsection{Stability}
\subsection{Graph Embedding}

==> tables/exmaple-bk.tex <==
\begin{table*}[t!]
\caption{Examples of semantically similar but syntactically different injection attacks on three languages}
\label{tb:exp}
\centering
\footnotesize
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccl}\toprule


%\textbf{Language}&\textbf{Injection Point}&\textbf{Injected Inputs}\\

%\midrule

\multirow{2}{*}{SQL}&injection point&\texttt{SELECT * FROM users WHERE username='\textcolor{blue!50}{\textbf{\$name}}' and password='\textcolor{blue!50}{\textbf{\$pass}}';}\\
&injection attack&\texttt{SELECT * FROM users WHERE username='\textcolor{blue!50}{\textbf{' OR '1'='1';}}\colorbox{pink}{\textcolor{blue!50}{\textbf{ --}}' and password='\textcolor{blue!50}{\textbf{abc}}';}}\\

\multirow{2}{*}{XML (XPath)}&injection point&\texttt{users[username/text()='\textcolor{blue!50}{\textbf{\$name}}' and password/text()='\textcolor{blue!50}{\textbf{\$pass}}']}\\
&injection attack&\texttt{users[username/text()='\textcolor{blue!50}{\textbf{' OR '1'='1}}\colorbox{pink}{\textcolor{blue!50}{\textbf{(:}}' and password/text()='\textcolor{blue!50}{\textbf{:)}}}']}\\


%PHP&\texttt{if (eval("return '\$pass' === 'retrivePassword($\backslash$"\$username$\backslash$")';"))}\\


\multirow{2}{*}{PHP}&injection point&\texttt{if (\textit{eval}("return '\$storedName' === '\textcolor{blue!50}{\textbf{\$name}}' \&\& '\$storedPass' === '\textcolor{blue!50}{\textbf{\$pass}}';"))}\\


&injection attack&\texttt{return \$storedName === '\textcolor{blue!50}{\textbf{' || '1'=='1';}} \colorbox{pink}{\textcolor{blue!50}{\textbf{//}}' \&\& \$storedPass === '\textcolor{blue!50}{\textbf{abc}}';}}\\



\bottomrule
\end{tabular}
%}
\centering
 \begin{tablenotes}
    \footnotesize
     \item the \textcolor{blue!50}{blue}/bold texts are the inputs from the user, where \textcolor{blue!50}{\textbf{\$name}} and \textcolor{blue!50}{\textbf{\$pass}} denote the variable of the username and password given by an user, respectively. The highlighted texts are what have been commented out by the injection.
    \end{tablenotes}
\end{table*}

==> tables/exp-example.tex <==
\begin{table*}[t!]
	\caption{Illustrative examples of the translated test inputs in \texttt{\textsc{DaNuoYi}}\textcolor{red}{The layout needs to be improved!}}
	\label{tab:example}
	\footnotesize
	\begin{tabular}{lll}
		\toprule
		\textbf{Type}&\textbf{Test input}\\
		\midrule
		from SQLi & \textcolor{blue}{\texttt{\rq /**/or/**/\lq 1\rq=\lq 1\rq -- }}                                                                                                                                \\
		to XSS   & \textcolor{blue}{\texttt{\textgreater{}\textless{}s\%43\%72\%49pt\textgreater{}\%61\%6c\%65\%72\%74\%28\%31\%29\textless{}/s\%43ri\%70\%74\textgreater{}\textless{}!--}}                            \\ \hline
		from SQLi &\textcolor{blue}{\texttt{ 0\&quot;test\&quot; = \&quot;test\&quot;}}                                                                                                          \\
		to HTMLi  &\textcolor{blue}{\texttt{ \textless{}\%61+\%68e\%72f=\&\#x6A;\&\#x61;\&\#x76;\&\#x61;\&\#x73;\&\#x63;\&\#x72;\&\#x69;\&\#x70;\&\#x74;\&\#x3A;jsString \%20\textgreater{}}} \\ \hline %...
		from SQL & \textcolor{blue}{\texttt{\lq)/**/\&\& not/**/false or(\rq}}                                                                                                                                              \\
		to PHPi   & \textcolor{blue}{\texttt{O:7:``Example”:1:\{s:3:``var”;s:10:``phpinfo();”;\}}}                                                                                               \\ \hline
		from SQLi &\textcolor{blue}{\texttt{ )/**/;select sleep (2) \#}}                                                                                                                         \\
		to SSi  &\textcolor{blue}{\texttt{ 0 ; sleep \%20 1 |}} \\ \hline                                                                                                                           
	\end{tabular}
\end{table*}
